TubeR: Tubelet Transformer for Video Action Detection

We propose TubeR: a simple solution for spatio-temporal video action detection. Different from existing methods that depend on either an off-line actor detector or hand-designed actor-positional hypotheses like proposals or anchors, we propose to directly detect an action tubelet in a video by simultaneously performing action localization and recognition from a single representation. TubeR learns a set of tubelet-queries and utilizes a tubelet-attention module to model the dynamic spatio-temporal nature of a video clip, which effectively reinforces the model capacity compared to using actor-positional hypotheses in the spatio-temporal space. For videos containing transitional states or scene changes, we propose a context aware classification head to utilize short-term and long-term context to strengthen action classification, and an action switch regression head for detecting the precise temporal action extent. TubeR directly produces action tubelets with variable lengths and even maintains good results for long video clips. TubeR outperforms the previous state-of-the-art on commonly used action detection datasets AVA, UCF101-24 and JHMDB51-21.

==> tex/5_vis.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{fig/fig3_1.png}
    \caption{Visualization of tubelet specific feature with attention rollout. Best view in color.}
    \label{fig:visualization}

\end{figure*}

\paragraph{Feature Visualization. } We first provide visualizations (Figure \ref{fig:visualization}) of the tubelet-specific features by overlay the tubelet-specific feature activation to the input frame using attention rollout \cite{abnar2020quantifying}. The example in Figure \ref{fig:visualization} is a challenge case as it contains multiple people and concurrent actions, the clip also has view occasion and scale changes. The visualization show that: 1. the proposed TubeR is able to generate highly discriminative tubelet-specific features. The four people in this case are clearly separated in different tubelets. 2. The action switch works as expected and initiate/cut the tubelets when the action starts/stops. 3. The TubeR generalize well to scale changes(the brown box). 4. The generated final tubelets are tightly associated with tubelet specific feature, which is as expected. 

\paragraph{Error Analysis. } 
We further visualize a few failed cases and discuss the limitation of TubeR.

